Quantum Crystals and Spin Chains

In this note, we discuss the quantum version of the melting crystal corner in one, two, and three dimensions, generalizing the treatment for the quantum dimer model. Using a mapping to spin chains we find that the two--dimensional case (growth of random partitions) is integrable and leads directly to the Hamiltonian of the Heisenberg XXZ ferromagnet. The three--dimensional case of the melting crystal corner is described in terms of a system of coupled XXZ spin chains. We give a conjecture for its mass gap and analyze the system numerically.

==> BetheDimer.tex <==

\section{Bethe ansatz for the quantum dimer on a hexagonal lattice}
\label{sec:bethe-ansatz-quantum}

The quantum dimer problem, as introduced by Rokhsar and Kivelson in
\cite{Rokhsar1988} is described by the Hamiltonian
\begin{equation}
  \label{eq:RK}
  \HH_{\text{dimer}} =  - J \sum\ketbra{\blacksquare}{\square} +  \ketbra{\square}{\blacksquare} + V \sum  \ketbra{ \square}{\square} +  \ketbra{ \blacksquare}{\blacksquare} \, ,
\end{equation}
where the states $\ket{\blacksquare}$ and $\ket{\square}$ represent
the two possible dimer configurations in an elementary cell. In
particular, in the case of the hexagonal lattice, one shows that the
possible configurations are in one--to--one correspondence with those
of the three--dimensional crystal melting. This means that we can use
the same description in terms of interacting spin chains and write the
Hamiltonian as
\begin{equation}
  \label{eq:3d-HamiltonianApp}
  \HH_{\text{dimer}}  =  \sum_{x \in \setZ} \sum_{ z \in \setZ + \frac{x+1}{2}} \HH_{\text{dimer}}^{(x,z) \to (x, z+1)} \left( 1- n_{x+1,z+1/2} \right) \left( 1 -  n_{x-1,z+1/2} \right) \, ,
\end{equation}
where
\begin{equation}
  \HH_{\text{dimer}}^{(x,z) \to (x, z+1)} = -J \left( \psi^*_{x,z+1} \psi_{x,z} + \psi^*_{x,z} \psi_{x,z+1} \right) + V n_{x,z} \left( 1 - n_{x,z+1} \right) + V n_{x,z+1} \left( 1 - n_{x,z} \right) \, .
\end{equation}
The quantum dimer problem is described by a sector of this spin chain
Hamiltonian, precisely the one obeying he conditions in
Eq.~(\ref{eq:3d-sector-conditions}).  Just like in the quantum
crystal, this problem can be studied via the Bethe
ansatz. Again consider the finite case, \ie\ the system in a box of
size $N \times N \times N$. In this case the relevant boundary
conditions are the so--called open ones in both the $z$ and $x$
directions.

Again we borrow the notation from~\cite{Alcaraz:1987}. An $n$--particle
eigenstate is written as
\begin{equation}
  \ket{\alpha } = \sum_{\mathbf{x},\mathbf{z}} f(x_1, z_1 ; \dots ; x_n,z_n) \ket{x_1,z_1; \dots; x_n,z_n} \, ,
\end{equation}
where $\mathbf{x}= \set{x_1, \dots, x_n}$, $\mathbf{z}= \set{z_1,
  \dots, z_n}$ and $\ket{\mathbf{x}, \mathbf{z}} $ describes the $n$
particles at position $(x_i, z_i)$.
The ansatz for the function $f(\mathbf{x},\mathbf{z}) $ is
\begin{equation}
  f ( \mathbf{x}, \mathbf{z} ) = \sum_P \epsilon_P A (x_{p(1)}, k_{p(1)}; \dots ; x_{p(n)}, k_{p(n)} ) e^{\imath \left( k_{p(1)} z_1 + \dots + k_{p(n)} z_n  \right) }\, , 
\end{equation}
where the sum runs over all permutations and negations of $k_i$, and
$\epsilon_P$ is the corresponding sign, which changes with each
transposition or negation. Note that since the motion happens only
along the $z$--axis, the problem remains essentially
one--dimensional. By the definition of an eigenstate, $\ket{\alpha} $
satisfies the equation
\begin{equation}
  \HH_{\text{3d}}^N \ket{\alpha} = E_\alpha \ket{\alpha} \, .  
\end{equation}
which translates into equations of the type
\begin{equation}
  f( x, z + 1 ) + f ( x, z - 1 ) - 2 \Delta f( x, z ) = E f(x,z) \, .
\end{equation}
In our formulation the Hamiltonian must be supplemented by the
boundary conditions which read for a single--particle state
\begin{equation}
  \label{eq:BoundaryBetheDimer}
  \begin{cases}
    f ( x, -N - \frac{ \abs{x} + 1 }{2} ) = V f ( x, -N - \frac{ \abs{x} - 1 }{2}  ), \\
    f ( x, N - \frac{ \abs{x} - 1 }{2}  ) = V f ( x, N - \frac{ \abs{x} + 1 }{2} ).
  \end{cases}
\end{equation}
Moreover, the particles, being fermions, cannot occupy the same point at
the same time, which results in the following scattering equation
for the two--particle state:
\begin{equation}
  f (x, z; x, z) + f( x, z + 1; x, z + 1 ) = 2\, V f (x, z; x, z + 1 ) \, .  
\end{equation}
The extra condition coming from the interaction between two adjacent
spin chains can be stated in a similar way in terms of scattering:
\begin{equation}
  f (x, z; x \pm 1, z- 1/2) + f( x, z - 1; x \pm 1, z + 1/2 ) = 2 \, V f (x, z; x \pm 1, z + 1/2 )   
\end{equation}
(note that two adjacent chains are shifted by $1/2$ in the $z$ direction).

Introducing the functions
\begin{align}
  \beta (k) &= \left( 1 - V e^{-\imath k}  \right) e^{\imath k \left( 2N +1 \right)} \,, \\
  s( k_1, k_2 ) &= 1 + e^{\imath \left( k_1 + k_2  \right) }- 2 V\, e^{\imath k_2} ,
\end{align}
we can define
\begin{align}
  \beta (x, k) &= \exp \left[ \imath k \left( -N  -\textstyle{\frac{ \abs{x} + 1 }{2}}  \right) \right] \beta (k) \, ,\\
  s(x_1, k_1 ; x_2, k_2 ) &=
  \begin{cases}
    s( k_1, k_2 ) & \text{ if $x_1 = x_2 $, } \\
    e^{-\imath k_2/2} s(k_1, k_2 ) & \text{ it $x_1 = x_2 \pm 1$,} \\
    1 & \text{otherwise.} 
  \end{cases}
\end{align}
It is then easy to show that
\begin{equation}
  A (\mathbf{x}, \mathbf{k}) = \prod_{j=1}^n \beta(x_j, -k_j) \prod_{1 \leq j < l \leq n} B( x_j, -k_j; x_l, k_l) e^{-\imath k_l} \, ,  
\end{equation}
where
\begin{equation}
  B (x_1, k_1 ; x_2, k_2 ) = s (x_1, k_1 ; x_2, k_2 )  s (x_2, k_2 ; x_1, - k_1 ) \, . 
\end{equation}
The energy is then given by
\begin{equation}
  E_\alpha = - J \sum_{j=1}^n \left( \cos k_j - V \right) \, ,  
\end{equation}
and the momenta satisfy the Bethe equations
\begin{equation}
  e^{2 \imath \left(2 N - 1 \right) k_j } \left( \frac{e^{\imath k_j} - V }{e^{-\imath k_j} - V }  \right)^2 = \prod_{\substack{l=1\\ l \neq j}}^n \frac{B(x_j, -k_j ; x_l, k_l)}{B(x_j,k_j; x_l, k_l)} \, .  
\end{equation}

The results of this calculations are clearly very close to those in
Sec.~\ref{sec:bethe-ansatz} once we identify $V$ and
$\Delta$. Actually, the only difference is found in the boundary
conditions that are of the kink type in
Eq.~(\ref{eq:BoundaryBetheCrystal}) and open in
Eq.~(\ref{eq:BoundaryBetheDimer}). The difference disappears for $V =
\Delta = q = 1$ where both the quantum crystal and the quantum dimer
describe the usual Rokhsar and Kivelson point for the hexagonal lattice
and, in fact, in this limit, the two Bethe ansätze coincide.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Draft2d"
%%% End: 


==> Strings.tex <==
\section{String theory realization}

We would like to connect our earlier findings to string theory, which leads us towards black hole physics. Seeking to deepen the understanding of the relation~\cite{Ooguri:2004zv}
\begin{equation}\label{OSV}
Z_{\text{BH}}=\left| Z^{\text{top}}\right|^2,
\end{equation}
it was shown in~\cite{Vafa:2004qa} that for a special class of geometries, namely for Calabi--Yaus $M$, where $M$ is the total space over the rank 2 vector bundle over the torus  
\begin{equation}
{\mathcal O}(m)\oplus{\mathcal O}(-m)\to T^2,\quad m\ \text{integer},
\end{equation}
that perturbative amplitudes of the topological string A--model match the large $N$ expansion for amplitudes of 2d bosonic $U(N)$ Yang--Mills theory on the two--torus. On the other hand, it was shown that the topological string theory amplitudes are related to the dual brane theory, which turns out to be four dimensional ${\cal N}=4$ topologically twisted Yang--Mills theory on a line bundle over $T^2$. Take type IIA string theory compactified on the Calabi--Yau $M$, where $M$ is the total space over the rank 2 vector bundle over the torus  ${\mathcal O}(m)\oplus{\mathcal O}(-m)\to T^2$. By wrapping appropriate numbers of D4--branes on $T^2$ and one of the complex fiber directions, D2--branes on $T^2$ and putting D0--branes, one obtains the brane field theory, a supersymmetric $U(N)$ gauge theory which corresponds to 4D charged black holes.

The circle of ideas in~\cite{Vafa:2004qa} was completed by showing that the topologically twisted brane theory reduces to a two dimensional topologically 
twisted theory on $T^2$ which in turn is equivalent to 2d bosonic Yang--Mills on $T^2$.  As discussed in~\cite{Dijkgraaf:2005bp}, the 2d bosonic  $U(N)$ Yang--Mills theory on a torus has a reformulation in terms of free fermions, which helps us to connect to our model.

The 2d system we have studied so far has a realization in string theory if one goes to a certain simplified limit. In fact, it corresponds to the case with linear dispersion relation given in~\cite{Dijkgraaf:2005bp}, which describes the large $N$ limit of 2d Yang--Mills. To capture the non--perturbative corrections for finite $N$, corresponding to the entanglement of the two Fermi surfaces of the free fermion system, a system with quadratic dispersion relation is studied in~\cite{Dijkgraaf:2005bp}. Its partition function is given by
\begin{equation}
\label{eq:quadratic}
 Z = \prod_{k\in \setZ + 1/2} \left( 1 + z^2 q^{k^2} y^k \right)\,.
\end{equation}


To go beyond the case with linear dispersion relation and to arrive at~(\ref{eq:quadratic}), we need to generalize the quantum Hamiltonian, which we will do in the following. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Free fermions with quadratic dispersion relation}

We want to describe a system of fermions with a quadratic dispersion
relation, whose ``classical'' partition function reads
\begin{equation}
  Z = \Tr ( e^{\imath \vartheta P + g_s E } ) = \Tr (q^{k^2} y^k ) \, ,  
\end{equation}
where
\begin{align}
  q = e^{-g_s}, && y = e^{\imath \theta} \, .
\end{align}
This describes a system of fermions on a 1d lattice of length $N$
which have the energies $E = \sum_i k^2_i$ and momenta $P = \sum_i k$.
Using the same construction as before we want to find a Hamiltonian
admitting the vector $\ket{\text{ground}}$ as a ground state with the
condition
\begin{equation}
  \braket{ \text{ground}| \text{ground} } = Z \, .  
\end{equation}

The simplest approach consists in this case in generalizing the
previous construction and introducing the following Hamiltonian:
\begin{equation}
  \label{eq:quadratic-quantum_Hamiltonian}
  \begin{split}
    \HH &= - J \sum_{k\in \setZ + 1/2} \psi_{k+1}^* \psi_k + \psi_k^* \psi_{k+1} - y^{1/2} q^{k+1/2} n_k \left( 1 - n_{k+1} \right) - y^{-1/2} q^{-k-1/2} n_{k+1} \left( 1 - n_k \right) = \\
    &= - \frac{J}{2} \sum_{k\in \setZ + 1/2} \sigma^1_k \sigma^1_{k+1} + \sigma^2_k
    \sigma^2_{k+1} + \Delta_k \sigma^3_{k} \sigma^3_{k+1} \, ,
  \end{split}
\end{equation}
where
\begin{equation}
  \Delta_k = \frac{1}{2} \left( y^{1/2} q^{2k+1} + y^{-1/2} q^{-2k-1} \right) = \cosh (\frac{\imath \vartheta + \left( 2 k + 1 \right) g_s }{2})  \, .
\end{equation}
A grand--canonical kink ground state can be introduced also in this case
and takes the form
\begin{equation}
\label{eq:grand-canonical-quadratic}
  \ket{\Psi(z)} = \prod_{k\in \setZ+1/2} \left( 1 + z q^{k^2/2} y^k \psi_k^* \right) \ket{0} = \sum_{N \in \setN} z^{2N} \Psi_N \ket{0} \, ,  
\end{equation}
where $\Psi_N \ket{0}$ is the ground state in the sector with $N$
spins up.
It is immediate to verify that
\begin{equation}
  \braket{\Psi (z) | \Psi(z)} = \prod_{k\in \setZ + 1/2} \left( 1 + z^2 q^{k^2} y^k \right),
\end{equation}
which is in fact the generating function for the partition functions
of systems with $N$ fermions.

To prove that the grand--canonical state in
Eq.~(\ref{eq:grand-canonical-quadratic}) is a zero--energy ground
state of the Hamiltonian~(\ref{eq:quadratic-quantum_Hamiltonian}) one
can generalize the construction presented in~\cite{Starr}. The
operator $\HH$ can be written as
\begin{equation}
  \HH = - J \sum_{k\in \setZ + 1/2} h_{k,k+1} \, ,
\end{equation}
where $h_{k,k+1}$ is the pojector on the state $\ket{\xi_{k,k+1}}$ defined by
\begin{equation}
  \ket{\xi_{k,k+1}} = \left(  y^{-1/4} q^{-k/2 - 1/4} \psi_{k+1}^*  - y^{1/4} q^{k/2 + 1/4} \psi_k^*  \right)  \ket{0_{k,k + 1}} \, ,
\end{equation}
where $\ket{0}_{k,k+1}$ represents two holes in $k$ and $k+1$. The
state $\ket{\Psi(z)}$ restricted to the points $k$ and $k+1$ reads:
\begin{equation}
  \ket{\Psi(z)_{k,k+1}} = \left( 1 + z\, q^{k^2/2} y^{k/2} \psi^*_k \right) \left( 1 + z\, q^{\left( k + 1 \right)^2/2} y^{\left( k + 1 \right)/2} \psi^*_{k+1} \right) \ket{0_{k,k+1}} \, , 
\end{equation}
so it is immediate to verify that
\begin{equation}
  \braket{ \xi_{k,k+1} | \Psi(z)_{k,k+1}} = 0 \, .
\end{equation}
This is of course true for each term in the sum, thus proving
\begin{equation}
  \HH \ket{\Psi(z)} = 0 \, . 
\end{equation}








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Draft2d"
%%% End: 

